Universality of Approximate Message Passing with Semi-Random Matrices

Approximate Message Passing (AMP) is a class of iterative algorithms that have found applications in many problems in high-dimensional statistics and machine learning. In its general form, AMP can be formulated as an iterative procedure driven by a matrix $\mathbf{M}$. Theoretical analyses of AMP typically assume strong distributional properties on $\mathbf{M}$ such as $\mathbf{M}$ has i.i.d. sub-Gaussian entries or is drawn from a rotational invariant ensemble. However, numerical experiments suggest that the behavior of AMP is universal, as long as the eigenvectors of $\mathbf{M}$ are generic. In this paper, we take the first step in rigorously understanding this universality phenomenon. In particular, we investigate a class of memory-free AMP algorithms (proposed by \c{C}akmak and Opper for mean-field Ising spin glasses), and show that their asymptotic dynamics is universal on a broad class of semi-random matrices. In addition to having the standard rotational invariant ensemble as a special case, the class of semi-random matrices that we define in this work also includes matrices constructed with very limited randomness. One such example is a randomly signed version of the Sine model, introduced by Marinari, Parisi, Potters, and Ritort for spin glasses with fully deterministic couplings.

==> Semi-random Universality ArXiv Final/commands.tex <==
% Common commands and definitions

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{latexsym}
\usepackage{verbatim}
%\usepackage{subfigure}
\usepackage[final]{graphicx}
\usepackage{psfrag}
\usepackage{mathrsfs}  
\usepackage{amsthm}
%\usepackage{xcolor}
\usepackage{fancybox}
\usepackage{enumitem}
%\usepackage{mathabx}
\usepackage[export]{adjustbox}
\usepackage{caption,subcaption}



\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}



\newenvironment{densitemize}%    Densely printed itemized list,
{\begin{list}               %    with flush left bullets.
    {$\bullet$ \hfill}{
        \setlength{\leftmargin}{\parindent}
        \setlength{\parsep}{0.04\baselineskip}
        \setlength{\itemsep}{0.5\parsep}
        \setlength{\labelwidth}{\leftmargin}
        \setlength{\labelsep}{0em}}
    }
{\end{list}}

\providecommand{\eref}[1]{\eqref{eq:#1}}  % call \eqref from amstex
\providecommand{\cref}[1]{Chapter~\ref{chap:#1}}
\providecommand{\sref}[1]{Section~\ref{sec:#1}}
\providecommand{\appref}[1]{Appendix~\ref{appendix:#1}}
\providecommand{\fref}[1]{Figure~\ref{fig:#1}}
\providecommand{\tref}[1]{Table~\ref{tab:#1}}
\providecommand{\thref}[1]{Theorem~\ref{thm:#1}}
\providecommand{\defref}[1]{Definition~\ref{def:#1}}
\providecommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\providecommand{\remref}[1]{Remark~\ref{rem:#1}}
\providecommand{\assumpref}[1]{Assumption~\ref{assump:#1}}
\providecommand{\factref}[1]{Fact~\ref{fact:#1}}
\providecommand{\propref}[1]{Proposition~\ref{prop:#1}}
\providecommand{\corref}[1]{Corollary~\ref{cor:#1}}

\providecommand{\R}{\ensuremath{\mathbb{R}}}
\providecommand{\C}{\ensuremath{\mathbb{C}}}
\providecommand{\N}{\ensuremath{\mathbb{N}}}
\providecommand{\Z}{\ensuremath{\mathbb{Z}}}
\providecommand{\W}{\ensuremath{\mathbb{N}_0}}


\providecommand{\bfP}{\mathbf{P}}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\inprod}[1]{\langle#1\rangle}
\providecommand{\set}[1]{\left\{#1\right\}}
\providecommand{\seq}[1]{\left<#1\right>}
\providecommand{\bydef}{\overset{\text{def}}{=}}
\renewcommand{\dim}{N}
\providecommand{\sigpsi}{\sigma_{\psi}^2}
\providecommand{\siglam}{\sigma_{\lambda}^2}

\renewcommand{\vec}[1]{\ensuremath{\boldsymbol{#1}}}
\providecommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}

% Some calligraphic letters
\providecommand{\calS}{\mathcal{S}}
\providecommand{\calP}{\mathcal{P}}
\providecommand{\calH}{\mathcal{H}}
\providecommand{\calM}{\mathcal{M}}
\providecommand{\calV}{\mathcal{V}}
\providecommand{\calF}{\mathcal{F}}
\providecommand{\calO}{\mathcal{O}}

% Common matrices and vectors
\providecommand{\mA}{\mat{A}} \providecommand{\mB}{\mat{B}}
\providecommand{\mC}{\mat{C}} 
\providecommand{\mD}{\mat{D}}
\providecommand{\mF}{\mat{F}}
\providecommand{\mH}{\mat{H}}
\providecommand{\mI}{\mat{I}} \providecommand{\mJ}{\mat{J}} 
\providecommand{\mK}{\mat{K}} \providecommand{\mL}{\mat{L}} 
\providecommand{\mM}{\mat{M}} \providecommand{\mP}{\mat{P}} 
\providecommand{\mQ}{\mat{Q}} \providecommand{\mR}{\mat{R}}
\providecommand{\mS}{\mat{S}} \providecommand{\mU}{\mat{U}} 
\providecommand{\mV}{\mat{V}}
\providecommand{\mW}{\mat{W}}
\providecommand{\mT}{\mat{T}}
\providecommand{\mZ}{\mat{Z}}
\providecommand{\mSigma}{\mat{\Sigma}}
\providecommand{\mGm}{\mat{\Gamma}} \providecommand{\mG}{\mat{G}}
\providecommand{\mPsi}{\mat{\Psi}}
\providecommand{\mPsi}{\mat{\Psi}}
\providecommand{\mX}{\mat{X}}



\providecommand{\va}{\vec{a}} \providecommand{\vb}{\vec{b}}
\providecommand{\vc}{\vec{c}} \providecommand{\ve}{\vec{e}}
\providecommand{\vg}{\vec{g}}
\providecommand{\vh}{\vec{h}} \providecommand{\vk}{\vec{k}}
\providecommand{\vm}{\vec{m}} \providecommand{\vn}{\vec{n}} 
\providecommand{\vl}{\vec{l}} \providecommand{\vp}{\vec{p}}
\providecommand{\vq}{\vec{q}} 
\providecommand{\vr}{\vec{r}}
\providecommand{\vs}{\vec{s}}
\providecommand{\vt}{\vec{t}}
\providecommand{\vu}{\vec{u}} \providecommand{\vw}{\vec{w}}
\providecommand{\vx}{\vec{x}} \providecommand{\vy}{\vec{y}}
\providecommand{\vz}{\vec{z}} \providecommand{\vi}{\vec{i}}
\providecommand{\vj}{\vec{j}} \providecommand{\vzero}{\vec{0}}
\providecommand{\vgm}{\vec{\gamma}} 
\providecommand{\vxi}{\vec{\xi}}
\providecommand{\vv}{\vec{v}}
\providecommand{\vomg}{\vec{\omega}}
\providecommand{\vell}{\vec{\ell}}
\providecommand{\vDelta}{\vec{\Delta}}
\providecommand{\valpha}{\vec{\alpha}}
\providecommand{\vbeta}{\vec{\beta}}
\providecommand{\vepsilon}{\vec{\epsilon}}
\providecommand{\vsigma}{\vec{\sigma}}
\providecommand{\fieldvec}{\vec{1}}
\providecommand{\fieldscal}{{s}}
\providecommand{\vone}{\vec{1}}



\providecommand{\w}{\omega}

\providecommand{\conv}{\ast}
\providecommand{\circonv}[1]{\circledast_{#1}}

%%% additional commands
\newcommand{\unif}[1]{\mathsf{Unif}(#1)} %% use for Haar measure/ Uniform measure
\newcommand{\ortho}{\mathbb{O}} %% use for orthogonal group
\newcommand{\explain}[2]{\overset{\text{\tiny{#1}}}{#2}}
\newcommand{\iter}[2]{{#1}^{(#2)}} %% use it to define iterates
\newcommand{\E}{\mathbb{E}} %% for expectations
\renewcommand{\P}{\mathbb{P}} %% for probabilities
\newcommand{\Var}{\mathrm{Var}}
\usepackage[numbers]{natbib} % for citet, citep etc
\newcommand{\sphere}[1]{\mathcal{S}^{#1}} % use for unit sphere
\newcommand{\ip}[2]{\left\langle {#1}, {#2} \right\rangle} %use for inner product
\newcommand{\Op}{\mathcal{O}_\mathsf{P}} %% for stochastic order notation
\newcommand{\gauss}[2]{\mathcal{N}\left( #1,#2 \right)} %% for Gaussian distribution
\newcommand{\nonlin}{f}

%% commands related to combinatorics
\newcommand{\degree}{D}
\newcommand{\fourier}[3]{\hat{\nonlin}_{#1}(#2,#3)}
\newcommand{\pweight}[1]{p_{#1}}
\newcommand{\qweight}[1]{q_{#1}}
\newcommand{\effect}[1]{\omega_{#1}}
\newcommand{\height}[1]{h_{#1}}
\newcommand{\valid}{\mathtt{VALID}}
\newcommand{\hermite}[1]{H_{#1}}
\newcommand{\trees}[2]{\mathscr{T}_{#1}(#2)}
\newcommand{\forests}[2]{\mathscr{F}_{#1}(#2)}
\newcommand{\colorings}[2]{\mathscr{C}_{#1}(#2)}
\newcommand{\pleaves}[1]{\mathscr{L}_{>0}(#1)}
\newcommand{\leaves}[1]{\mathscr{L}(#1)}
\newcommand{\nullleaves}[1]{\mathscr{L}_0(#1)}
\newcommand{\enodes}{\mathscr{E}}
\newcommand{\gnodes}{\mathscr{G}}
\newcommand{\onodes}{\mathscr{O}}
\newcommand{\bnodes}{\mathscr{B}}
\newcommand{\eleaves}{\mathscr{L}_e}
\newcommand{\gleaves}{\mathscr{L}_g}
\newcommand{\tileaves}{\mathscr{L}_1}
\newcommand{\tiileaves}{\mathscr{L}_2}
\newcommand{\tiiileaves}{\mathscr{L}_3}
\newcommand{\nleaves}{\mathscr{L}_0}
\newcommand{\map}{\mathscr{M}}
\renewcommand{\part}[1]{\mathscr{P}(#1)}
\newcommand{\chrn}[1]{c_{#1}}
\newcommand{\wcolorings}[2]{\mathscr{WC}_{#1}(#2)}
\newcommand{\mobius}[2]{\mu(#1, #2)}
\newcommand{\rootset}{\mathscr{R}}
\newcommand{\gibbs}{\mu_{\dim}}
\newcommand{\temp}{\beta}
\newcommand{\field}{\theta}
\newcommand{\invpoly}{\Gamma}
\newcommand{\universal}{simple }
\newcommand{\exponent}{\eta}
\newcommand{\intuition}[1]{{\color{blue}#1}}
\newcommand{\mgnt}{\chi}
\newcommand{\vmgnt}{\vec{\mgnt}}
\newcommand{\pw}{$\mathrm{PW}_2$}


\makeatletter
\newcommand{\myitem}[1]{%
\item[#1]\protected@edef\@currentlabel{#1}%
}
\makeatother

\makeatletter
\newenvironment{tagsubequations}[1]
 {%
  \addtocounter{equation}{-1}%
  \begin{subequations}
  \renewcommand{\theparentequation}{#1}%
  \def\@currentlabel{#1}%
 }
 {%
  \end{subequations}\ignorespacesafterend
 }
\makeatother


%%%% for algorithms
%%% for algorithms

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}

%% code for widecheck
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\DeclareMathAccent{\wideparen}{0}{mathx}{"75}

\def\cs#1{\texttt{\char`\\#1}}
%%%%%%%
\providecommand{\ctr}[1]{\widecheck{#1}}

